Understanding blockchain: definitions, architecture, design, and system comparison

The explosive advent of the blockchain technology has led to hundreds of blockchain systems in the industry, thousands of academic papers published over the last few years, and an even larger number of new initiatives and projects. Despite the emerging consolidation efforts, the area remains highly turbulent without systematization, educational materials, or cross-system comparative analysis. In this paper, we provide a systematic and comprehensive study of four popular yet widely different blockchain systems: Bitcoin, Ethereum, Hyperledger Fabric, and IOTA. The study is presented as a cross-system comparison, which is organized by clearly identified aspects: definitions, roles of the participants, entities, and the characteristics and design of each of the commonly used layers in the cross-system blockchain architecture. Our exploration goes deeper compared to what is currently available in academic surveys and tutorials. For example, we provide the first extensive coverage of the storage layer in Ethereum and the most comprehensive explanation of the consensus protocol in IOTA. The exposition is due to the consolidation of fragmented information gathered from white and yellow papers, academic publications, blogs, developer documentation, communication with the developers, as well as additional analysis gleaned from the source code. We hope that this survey will help the readers gain in-depth understanding of the design principles behind blockchain systems and contribute towards systematization of the area.

==> sections/application.tex <==
 \subsection{Application Layer}
 \label{sec:application}
 
Bitcoin can be viewed as a final application by itself, with limited extensibility through scripting. At the same time, Ethereum and Hyperledger Fabric can be regarded as platforms for application development on top of them. Beside cryptocurrency management, public Ethereum deployment is more suited for developing large-scale public B2C applications implemented via smart contracts.  Private Ethereum and Fabric are designed as a platform for B2B applications implementing business agreements within a consortium, such as managing the logistics for a large supply chain or sharing the data that is subject to access restrictions.
It would be interesting to survey different Ethereum and Fabric applications and categorize them with the purpose of gaining deeper insight. This effort is orthogonal to the goals of this survey.
 
% In contrast to the Bitcoin blockchain system which is used mainly for exchanging Bitcoin cryptocurrency, Ethereum, Hyperledger Fabric, and IOTA can be used for executing more variety of applications. 
 
% Beside exchanging cryptocurency, public Ethereum is more suited for developing B2C applications by the help of the smart contracts. As public Ethereum is a permissionless blockchain, participants are free to join the network and use the public application. Private Ethereum and Hyperledger Fabric are designed as a platform for B2B applications. As an example of a B2B model of blockchain application, smart contracts can be used for transferring digital products from one company to another by executing a transaction automatically under a given condition. 
 
The IRI version of IOTA covered in this survey is not extensible either, though newer versions of IOTA in development provide a number of extensions.  
%This also applies to IOTA IRI even 
These extensions are geared towards the Internet of Things (IoT) industry~\cite{iot} and put emphasis on low computational load and energy consumption. Some of these extensions aim at B2B models~\cite{iotab2b}.
%IOTA provides secure communications for the involved IoT devices. In addition to the IoT functioning, IOTA can also become handy in B2B models~\cite{iotab2b}.    


==> sections/extension.tex <==
\section{Blockchain as an Extension of Bitcoin}
\label{sec:blockchainasan}

Bitcoin as the first implementation of the chain of blocks concept is still working successfully in the context of cryptocurrency. Gradually, from the manifestation of bitcoin, different blockchain systems has been appeared and has extended the concept of blockchain introduced in bitcoin in order to apply its functionalities and advantageous properties of Section \ref{sec:properties} to broader contexts. In this section, first, the general model of blockchain systems according to their different requirements will be introduced. Then, the extended functionalities which could be applied to the blockchain systems are discussed. Finally, multiple implementation solutions for satisfying the functional and non-functional requirements will be mentioned.

\subsection{General Model}
\label{sec:model}
Different use cases of blockchain are not similar according to the requirements of non-functional properties. The model that bitcoin presents for non-functional properties such as scalability, performance, privacy, trust, and authorizaton may not be applicable to the other use cases of blockchain systems.

\begin{description}
\item[Scalability] Bitcoin scales to million users but only allows seven transactions per second.

\item[Performance]

\item[Privacy]

\item[Trust]

\item[Authorization]

\end{description} 

\subsection{Extended Functionality}
\label{sec:extended}
In order to achieve a blockchain system beyond cryptocurrencies, it is needed to extend the functionalities introduced by bitcoin. Smart contract and business logic are the main extensions of bitcoin that provide more functionalities in various contexts for blockchain systems.

\begin{description}
\item[Smart Contract]

\item[Business Logic]

\end{description} 
 

\subsection{General Implementation Solutions}
\label{sec:impsolutions}
There are general implementation solutions for the functional and non-functional requirements of different use cases. Each of the solutions are applied to a particular layer of the blockchain architecture in order to satisfy the requirements of the use case.

\begin{description}
\item[Hardware]

\item[Data Storage]

\item[Communication]

\item[Data Manipulation]

\item[Contract]

\item[Application]
\end{description} 


==> sections/future.tex <==
\section{Outlook toward the future}
\label{sec:future}

In the previous sections, we have compared and analyzed the building blocks of four popular blockchain systems through our proposed layered framework. In this section, we discuss the ways that each of the four considered blockchain system can evolve in each layer in the future (see Table~\ref{tab:gaps}).

\begin{description}
\item[Hardware:] As Bitcoin hardware layer is dependent on ASICs for solving cryptopuzzles, new generation of ASCIs with increasing hash rates per seconds will definitely be a future evolution for Bitcoin. Besides, it is needed for the Bitcoin hardware layer to improve power efficiency during computations. On the other hand, with regard to the Ethereum dependency on GPU instead of ASICs, there is an uncertain future for new generation of GPUs with higher memory bandwidth due to the switch from PoW to PoS in the next generations of Ethereum. In Hyperledger Fabric, FPGA based frameworks can be evolved to optimize the storage of data ledger and improve the security offered by TEE systems as well. At the end, IOTA needs to support for binary-based processors for industry adaptability reasons.

\item[Data storage:] Horizontal scalability techniques such as sharding protocol solutions~\cite{sharding} can be evolved in Bitcoin and Ethereum to solve the problem of ever increasing data storage per node. Elastico~\cite{elastico}, Omniledger~\cite{omniledger}, and Rapidchain~\cite{rapidchain} are a few examples of sharding solutions. Horiziontal scaling solutions in permissioned blockchains has also been proposed in some research like~\cite{horizontal}. However, as Hyperledger Fabric needs to focus more on maximizing transactions throughput in presence of more participants, some data storage solutions can be presented for resolving read-write set conflicts during the updates of concurrent transactions to the ledger. In IOTA, introducing local snapshots for pruning transaction history instead of the current centralized controlled snapshots can make the IOTA network independent of central authorities.

\item[Communication:] Construction of overlay network to maximize the transactions throughput is a communication layer solution for both Bitcoin and Ethereum. The idea of this kind of solutions is moving as much transaction off the main chain as possible. While the Lightning network~\cite{lightning} in Bitcoin is limited to work strictly for payments, Plasma~\cite{plasma} extends the idea to more complex computations, like Ethereum smart contracts. Hyperledger Fabric needs novel deterministic consensus algorithms to minimize the communication overhead between large scale of validating peers. Finally, IOTA, in its next releases, is shifting to a secure peer discovery mechanism, called Mana~\cite{coordicide}, based on reputation of nodes. 

\item[Data manipulation:] There are multiple observations for the future evolution of Bitcoin data manipulation layer. Increasing transaction throughput by introducing new soft forks such as Segwit~\cite{segwit}, safe blockchain configuration updates to reduce the risk of chain splits~\cite{}, and finding new incentivization methods for miners when the mining rewards reach to zero are some of the possible future works in data manipulation layer of Bitcoin. Reducing mining complexity by switching from PoW to PoS is an achievement in the next generation of Ethereum. In addition, Ethereum needs some solutions for safe blockchain configuration updates for the same purpose as Bitcoin. Mitigating performance bottleneck of endorsement phase and ordering phase of consensus in Hyperledger Fabric is a potential area of future research in data manipulation layer. IOTA plans to remove the role of central Coordinator and introduce a fully decentralized consensus protocol in its Coordicide release~\cite{coordicide}.     

\item[Contract] Enhancing the capabilities of Bitcoin scripts similar to Ethereum smart contracts can be a future evolution for Bitcoin contract layer. On the hand, enhancing the security of smart contracts against novel threat models is more important for the future of Ethereum and Hyperledger Fabric smart contracts. As IOTA lacks utilizing smart contracts, providing support for smart contracts can be an outlook toward the future of IOTA contract layer.  
\end{description}

\begin{table}
\centering
\tiny
\caption{Future Evolution of Layers of the Blockchain Systems}
\begin{tabular}{|p{1.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}|} 
 \hline
 \textbf{Blockchain Layer} & \textbf{Bitcoin} & \textbf{Ethereum} & \textbf{Hyperledger Fabric} & \textbf{IOTA} \\
  \hline
Hardware & New generation of ASCIs \& improving power efficiency~\cite{}  & Uncertain future due to the switch from PoW to PoS~\cite{}  & FPGA based frameworks~\cite{}  & Support for binary-based processors~\cite{} \\ 
 \hline
Data Storage & Sharding protocols & Sharding protocols & Resolving read-write set conflicts & local snapshots \\
 \hline 
Communication & Lightning network & Plasma  & Horizontal scaling, Minimizing the communication overhead between large scale of validating peers  & Mana \\
  \hline
Data Manipulation & Increasing transaction throughput, Safe blockchain configuration updates, \& Finding new incentivization methods for miners & Reducing mining complexity by switching from PoW to PoS \& Safe blockchain configuration updates & Mitigating performance bottleneck of endorsement phase and ordering phase of consensus & Fully decentralized consensus protocol \\ 
 \hline
 Contract & Enhancing scripts capabilities & Enhancing smart contracts' security  & Enhancing smart contracts' security & Provide support for smart contracts   \\ 
  \hline
 
\end{tabular}
\label{tab:gaps}
\end{table}

Additionally, we identify several open key technical challenges and possible directions for research towards the full adoption of blockchain systems to mainstream applications in industry. 

%\subsection{Decentralized Identity Management}
%The centralized~\cite{} and federated identity management solutions~\cite{} have been primarily dominating the digital identity industry since the dawn of the Internet. One of the fundamental drawbacks of these two models is that the central control of identity has never been with the user~\cite{}. The issuer and the verifier of the identity have had the central control of identity than the user.  

%With the advent of blockchain technologies, the possibilities of individuals gaining the control over their identities without the intervention of any centralized authorities have emerged. As a consequence, the notion of decentralized digital identity management has caught significant attention in industry~\cite{}, academia~\cite{}, and government agencies~\cite{}, leading to the development of new standards such as Verifiable Credentials (VCs)~\cite{} and Decentralized Identifiers (DIDs)~\cite{}. 

%One of the practical adoption difficulties for a decentralized digital identity management system is in the domain of providing digital services to children in public and private sectors. This difficulty arises due to the challenges involved in satisfying the requirements of compliance regulations~\cite{}. For example, one of the common compliance requirements across the world is to obtain parental/guardian consents to collect data from children~\cite{}{}{}. And, the age requirements for defining the individual as minor/child that need consent differ from a member state to another in the EU~\cite{}. 

%In this context, the decentralized identity management system requires to capture the family/guardian relationships between the decentralized identities and determine the age criteria for obtaining the consent specific to the geographical context. Furthermore, the relationship between the identities and the consents should be kept confidential following the privacy by design requirements. 

%To this end, identity management systems need to address the following challenges in a decentralized p2p environment before it can provide services to children/minors: 
%\begin{itemize}
%\item	How to effectively capture, store, retrieve and validate  the relationship between the permanent identifiers of entities such as parent/guardian and child such that the scalability and performance needs are addressed?
%\item	How to effectively capture, store, retrieve and validate the actions (such as consents) that are based on the identifiers’ relationships such that the scalability and performance needs are addressed?  
%\item	How to effectively maintain confidentiality regards to the relationship between the identities against the nodes in the large scale P2P?  
%\item	How to effectively maintain confidentiality on the actions that are built on top of the identifiers’ relationships against the nodes in the large scale P2P? 
%\item	How to enforce geographic-specific rules (such as determining the age criteria for requiring consent) to the nodes of P2P?
%\item	How to leverage the geographic-specific rules for the construction of the overlay networks to relay messages between the peers?   
%\end{itemize}

%The projects such as Hyperledger Indy (core decentralized identity features), Hyperledger Aries (core P2P infrastructure), Hyperledger URSA

%The research in the area of decentralized identity management is yet to fully address the above research challenges. As a consequence, any public block-chain systems using the decentralized identity management layer may not be able to offer compliant services to children in public and private sectors until the above mentioned challenges are addressed. 


\subsection{Interoperability between Blockchain Systems}
With the ongoing proliferation of blockchain systems tailored to the needs of different use cases~\cite{}, there is a crucial need for building interoperable solutions between the blockchain systems. Interoperability is the ability of blockchain systems to interact, coordinate, and cooperate with other blockchain systems. Interoperability solutions offer the following functionalities to blockchain systems~\cite{}: assets portability,  where assets from one blockchain system can be securely moved to another blockchain systems; atomic swap, where the assets can be swapped between two blockchain systems guaranteeing that either both transfers happen or neither of the transfer happens; cross-chain oracles, where a smart contract in local blockchain system can read the data from remote blockchain system and performs some action on the local blockchain systems; cross-chain asset encumbrance where assets are locked on the local blockchain system and the locking conditions are dependent on events on the remote blockchain system. 

Furthermore, Interoperability solutions that provide the above functionalities can be classified into three kinds~\cite{}: notary schemes, relays, and hash-locks. Notary schemes involve a trusted third party between two blockchain systems and have the potential to offer all the four functionalities through intermediate blockchain systems between the two blockchain systems. Hence, a single transaction may require state changes at three ledgers (sender, intermediate, and receiver). The trusted third party may introduce additional transaction fees for providing interoperable solutions. Examples of Notary schemes are Cosmos~\cite{} and 
Polkadot~\cite{}. 


Unlike Notary schemes, relays do not depend on a trusted third party and enable two blockchain systems to communicate with each other directly.  Relay based solutions can be further classified into one-way and two-way schemes. In the one-way scheme, a blockchain system X can read from another blockchain system Y, but the vice versa is not possible. An example is the BTC-relay~\cite{}, where the Bitcoin light client is running within the smart contract in Ethereum to verify transactions in Bitcoin through the block headers. Any node can act as a relay and submit block headers from Bitcoin to the BTCRelay smart contract in Ethereum. Scripts in Bitcoin are not sophisticated enough to run Ethereum clients to verify Ethereum transactions. As a consequence, the one-way relay does not provide atomic swaps functionality. 

In two-way relays, a blockchain system X can read from blockchain system Y, and vice versa is possible. Two-way relay solutions provide all the four functionalities. An example is the Dogethereum bridge~\cite{}, which would allow parties to lock a DOGE coin on the Dogethereum blockchain system to receive ERC20 token~\cite{} from Ethereum. And, the ERC 20 token owner in Ethereum can unlock the DOGE coin on the Dogethereum blockchain. Dogethereum bridge uses the concept of superblocks, which is a collection of all Dogecoin block headers collected in the last hour and merged into a Merkle tree. As a result, a delay of one hour is introduced in finalizing the transaction while minimizing the cost of verifying the blocks. Other examples of two-ways include PeaceRelay~\cite{} and Waterloo~\cite{}. 

The final scheme is hash-lock, where both the parties of the blockchain systems lock their tokens. The locks can be unlocked by the other party through sharing the pre-image of a hash. The sharing of the pre-image can be achieved through zero-knowledge proofs between the parties~\cite{}. Variants of hash-lock schemes are proposed~\cite{}, analyzed~\cite{} and surveyed~\cite{} in the literature. Hash-lock schemes are known to provide only atomic swaps functionality. 

Furthermore, all the three schemes focus mainly on solutions connecting two or more of the same type (public or private) of blockchain systems. The interoperability solutions connecting public and private blockchains still have the following open questions for future research.
 \begin{itemize}
\item	The public blockchain uses a probabilistic consensus protocol to update the states of the ledger. The private blockchain uses a deterministic consensus protocol to update the states of the ledger. When these two types of blockchains collaborate, how to ensure the finality of transactions, and how to provide atomic swaps functionality?

\item The throughput is relatively very low in public blockchains in compared to the private blockchains.  How to make sure that the throttling does not happen in public blockchains when transactions in private blockchains are sent to public blockchains?

\item How can the compliance policies of private blockchains be preserved during the collaboration? 

\item What are the new security attacks possible during the collaboration, how such attacks can be mitigated, and what are the trade-offs in the mitigation solutions? 

\end{itemize}

\subsection{Sharded blockchains}

One of the solutions that has been proposed for improving scalability of blockchain systems is sharding~\cite{sharding}~\cite{soksharding}~\cite{towardssharding}. Sharding in blockchain technology means splitting the entire blockchain resources including communication, computation, and storage, into separate partitions called $shards$ or $committees$. Partitioning communication, computation, and storage improves scalability by reducing the data communication overhead, maximizing the throughput of processed transactions, and reducing the disk storage size per node in the network. Permisstionless blockchain systems are more vulnerable to the scalability issues compared to permissioned blockchains because of the network size and decentralized management mechanism. Therefore, most of the sharding solutions such as Elastico~\cite{elastico}, Omniledger~\cite{omniledger}, Rapidchain~\cite{rapidchain}, and Chainspace~\cite{chainspace} have been proposed for permissionless blockchains. In addition to these recent research, Zilliqa~\cite{zilliqa} project is introduced in industry as another permissionless sharded blockchain to increase the number of transactions processed per second by dividing the
mining network into smaller consensus groups each capable of processing transactions in parallel. However, some aspects of sharding are implemented in permissioned blockchains as well; for example, Red Belly Blockchain~\cite{rbbc} assigns, for each group of transactions, distinct groups of proposer and verifier nodes, or RSCoin~\cite{rscoin} specifies distributed sets of authorities collecting valid transactions for its central bank.

The following steps are commonly followed in the implementation of the aforementioned permissionless sharded blockchains, though, each system may implement each step differently: 

 \begin{description}
\item[1) Committee formation:] The first step is distributing blockchain nodes to specific shards (committees). This distribution should be performed uniformly to have majority of honest nodes in each committee with high probability. For this uniformly distribution, the identity of the nodes are decided by solving a puzzle which is based on a randomness generation method. The main reason of using a randomness generation method is to make the puzzle unpredictable for attackers. Predictable puzzle weakens the security as the attacker have enough time to precompute the puzzle and target a specific result. In addition to be unpredictable, a good randomness generation method should generate public-verifiable and bias-resistance results~\cite{soksharding}. Public-verifiable result lets all of the participants verify the generated value, and bias-resistance feature prevents any participant to influence the result to its own advantage. Furthermore, none of the participants should be able to prevent the randomness generation progress, which makes availability as another important feature of the randomness generation method~\cite{soksharding}. After dedicating random generated identities to the nodes, they are assigned to the corresponding committees based on their identity.
 
Even though, the state-of-the-art work \cite{towardssharding} \cite{elastico} \cite{omniledger} \cite{rapidchain} proposes equations to indicate that the majority of the nodes in a committee should be honest for security reasons, the impact of the committee formation with respect to computation, communication, and storage overheads is overlooked.
 
\item[2) Overlay setup in committees:] After committee formation, overlay setup is needed for each committee. There should be mechanisms for tolerating inconsistent view of membership due to the decentralized nature of blockchain. Group membership protocols are running inside each shard to make sure that a consistent view of the network between the committee members is maintained. 

Two approaches are mostly used in the related works for overlay setup in each committee. One is utilizing a directory committee, like what is deployed in Elastico and ZIlliqa, which knows all of the committee members, and a node receives information of its peer by contacting the directory committee first. The second approach, that can be seen in Rapidchain, is using a peer discovery algorithm for each node to gossip its information to all of the committee members. The first approach has the complexity of generating a trusted directory committee, however, it has fewer communication overhead through the network than the second approach. In addition considering fault tolerance of the directory committee is another main challenge of the first approach.   

\item[3) Inter-committee communication (cross-shard):] Each committee is responsible for maintaining a disjoint set of transactions, but it may be needed to communicate with other committees to verify a transaction. These kind of transactions, validation of which are dependent on one or more transactions in another committees, are called cross-shard or global transactions. Two main approaches existing in the related works are utilizing user-driven protocols or deploying inter-committee routing protocols. In the user-driven protocols, example of which exists in Omniledger, the one who creates the transaction has the responsibility of gossiping and collecting the verifications from different committees. However, in the later approach deployed in Rapidchain, the transaction creator relies on a committee's leader which utilizes an inter-committee routing protocol to communicate with fewer number of committees for routing the transaction to the corresponding committee. In this approach, honest behaviour of the committee's leader becomes important as well as the routing algorithm efficiency. 

Cross-shard transactions suffer from longer confirmation time, and extra bandwidth consumption and computation cost; therefore, OptChain~\cite{optchain} has proposed a solution for minimizing cross-shard transactions. In contrary to the related works which randomly distribute arrival transactions to the committees, OptChain uses smart transaction placement method to group related transactions into the same shards to prevent further cross-shard verifications. Optchain deploys this solution as a user-side software which means that a transaction creator needs to monitor its own transactions as well as the information on the loads and confirmation time at the shards to make decision on which is the best shard to submit transactions. Although this approach minimizes cross-shard transactions, it will bring  computation costs for the transaction creator regardless of its honesty.        

\item[4) intra-committee consensus protocols:] After verifying all of the transactions in a block, committee members need to participate in an intra-committee consensus protocol to append the block into their blockchain. Despite increasing the throughput, sharding decreases security because fewer mining power is needed in each shard to perfom 51\% attack. Due to this security issue, BFT based consensus protocols are preferred to PoX-based ones, e.g. PoW or PoS, in sharded blockchains, however, they have the scalability issue. The ratio of faulty nodes in each committee should not exceed a threshold specified by the consensus protocol. Therefore, each of the related works deploys a modified implementation of BFT to improve fault tolerance of its committees. For example, Rapidchain increases the fault tolerance of intra-consensus protocol up to 50\% by its consensus protocol called $50\% BFT$~\cite{rapidchain}, nevertheless, it can only suit small-sized committees. As another example, Omniledger achieves low failure probability of the intra-consensus protocol by combining PoW and BFT algorithms in its ByzCoinX consensus protocol (an optimized version of ByzCoin~\cite{byzcoin}) at the cost of latency.  
 
\item[5) Data interleaving:] Data interleaving step includes mixing data collected from the shards in an orderly fashion in a separate chain outside the shards. Some of the related works such as Elastico and the future release of Ethereum (Ethereum 2.0~\cite{ethereum2}) have introduced an additional blockchain, called global blockchain, above the shards to facilitate communication between the shards. In this approach, there are two layers of consensus protocol exist towards ordering the transactions and blocks. The first one is the consensus protocol inside each committee happens in the previous step (intra-committee consensus), and the second layer of the consensus protocol is conducted by an additional global committee which computes a final result from all the values received from the shards. To do so, members in this global committee run another consensus protocol to agree on the final result to append it into the global blockchain, and broadcast the update to the network. On the contrary, in systems like Omniledger and RapidChain, there is only one consensus protocol (intra-committee), and a transaction is recorded only in one committee. Although, data interleaving step is reducing the complexity of data verifications in the shards, it can lead into another type of complexity which is consuming additional time and effort for building a consistent global blockchain in addition to the shards' local blockchains. 
 
\item[6) Epoch reconfiguration:] For the sake of security, the committee formation is dynamically changed based on time. Each period of time with a single committee formation is called an $epoch$. Epoch reconfiguration is done dynamically at the final step of each epoch to reconfigure the committees' formation. Similar to the committee formation, the epoch reconfiguration is performed based on a randomness generation method in order to prevent targeting or over taking a specific shard by faulty nodes. Two strategies used for dynamic reconfiguration are full swap and rolling. In full swap reconfiguration used in Elastico, all of the committees' formations are regenerated. However, in rolling strategy deployed in Omniledger and Rapidchain, multiple members of committees are swapped out and replaced with new members. The later strategy performs in a faster pace, though, it needs more attention for preserving the ratio of faulty nodes in rolling. Eventhough, epoch reconfiguration provides protection against adversary attacks due to the long term membership, it brings some challenges such as renewing the members database and the delay of the new nodes bootstrapping times. 

Currently, all of the sharded blockchian techniques perform epoch reconfiguration based on time. However, epoch reconfiguration can be triggered event-based by reaching some threshold conditions. Assume a condition in which the performance of the system is decreased due to the increased number of adversary nodes in a specific committee. In such a condition, triggering the epoch reconfiguration immediately, instead of waiting for the end time of the epoch, can prevent adversary nodes from further attacks in the targeted committee. Optimization objectives such as throughput of the number of transactions in a committee, committee members' storage size, or intra-committee consensus latency can be defined to trigger the epoch reconfiguration based on reaching the objectives' limits.
\end{description}

Despite all of the improvements conducted in each step of the current sharded blockchains, the following open questions for future research are still remained:

 \begin{itemize}
%general
\item For a blockchain system, $safety$ means that honest nodes agree on the same transaction/block, and $liveness$ is eventually reaching a consensus on a transaction/block. Then, how should a blockchain developer introduce sharding to an existing blockchain system such that safety and liveness are not being violated?
\item Before applying to the blockchain systems, sharding techniques had been used in other contexts such as databases to achieve scalability~\cite{spanner}~\cite{bigtable}. To what extent the traditional sharded database techniques are applicable to the blockchain systems?
%step 1 
\item Is there any distributed randomness generation mechanism which provides public-verifiability, bias-resistance, unpredictability, and availability at the same time in a proper time for a fast committee formation?
\item Currently, all of the related works in sharded blockchain systems are using a random assignment committee formation. Can we propose a smart committee formation solution instead of random assignment which provides maximum throughput of handling transaction, minimum latency of consensus and cross-shard transactions, and minimum storage complexity needed per node at the same time without jeopardizing the security of the system?
%step 3
\item Transaction atomicity in sharded blockchains means that the participants agree on committing or aborting the transaction, but not both~\cite{soksharding}. Is there any technique that can guarantee cross-shard transactions atomicity when shards do not trust each other?
%step 4  
\item Is there any technique that allows different shards use different consensus protocols according to their number of members? Then, what would be the impact of such a solution on the consensus layer of the overall blockchain?
%step 5
\item According to the sharded blockchains which are using an additional global blockchain for storing transactions, is there any solution for not loosing transactions and their outputs created in committees while the global blockchain is updating and broadcasting the updates to the committees?
%step 6
\item Is there any safe technique for reconfiguring the committees such that safety and liveness properties are not being violated? For example, no pending transactions get lost due to the committee members' swapping.  
\item When is the most appropriate time for the epoch reconfiguration? How often should it be performed? How do the optimization objectives of a committee impact the epoch reconfiguration time? 

\end{itemize}


%\begin{table}
%\centering
%\caption{A comparison of features' availability in representative blockchain systems}
%\resizebox{\textwidth}{!}{\begin{tabular}{|p{3cm}|p{1.5cm}|p{1.5cm}|p{3.2cm}|p{1cm}|} 
% \hline
% \textbf{Features} & \textbf{Bitcoin} & \textbf{Ethereum} & \textbf{Hyperledger Fabric} & \textbf{IOTA} \\
%  \hline
% Parental controlled accounts for minors & - & - & - & - \\ 
% \hline
%Wallet as proposer & - & - & - & \checkmark \\
% \hline 
%Remote PoW & - & - & - & \checkmark \\
%  \hline
%Database deletion & - & \checkmark & \checkmark & \checkmark \\ 
% \hline
% Centralized administration& - & - & \checkmark & \checkmark \\ 
%  \hline
%Scalability of consensus protocol & \checkmark & \checkmark & - & \checkmark \\ 
% \hline
% Deterministic consensus & - & - & \checkmark & - \\ 
% \hline
%  Native support for event emission & - & \checkmark & \checkmark & \checkmark \\
%  \hline
%  Configuration updates as transactions & - & - & \checkmark & - \\
%  \hline    
%\end{tabular}}
%\label{tab:gaps}
%\end{table}

%\begin{description}

%\item[Notion of accounts:] The notion of accounts are quite different in each of blockchain systems. Bitcoin lacks the concept of accounts, it uses unrelated Bitcoin addresses for receiving and sending bitcoins. On the other hand, Ethereum and Hyperledger Fabric exploit the notion of accounts to maintain and retrieve the recent states, assets and contracts easier and faster without needing to traverse the chain back and executing the transactions again to calculate the states. IOTA uses multiple accounts for each seed. Every seed in IOTA has three types of accounts associated with it. These accounts are Security Level 1, Security Level 2, and Security Level 3 providing different security levels according to the user's requirement. Each of these accounts can have multiple addresses. Although there is an improvement in IOTA in terms of adding security levels to the accounts, still we do not have relationship between accounts. For example, introducing the concepts of parent account and child account can provide linking between accounts and introduce more permission settings for them.  
%
%\item[Notion of wallets:] While wallets in Bitcoin and Ethereum are only used to facilitate storing and sending cryptocurrencies, and in Hyperledger Fabric, it contains a set of user identities, IOTA wallets adds more functionality than being a storage. IOTA has shown that wallets can have more responsibilities than what we have in Bitcoin and Ethereum. In addition to gathering and sending IOTA tokens, IOTA wallets contribute in the process of validating transactions, solving PoWs, and creating the bundles which make wallets more than a simple storage in IOTA systems. 
%
%\item[PoW responsibility:] In contrary to Bitcoin, Ethereum, IOTA has Shifted the responsibility of PoW from miners of the network to the client. In such a case, if mobile devices are going to do PoW then it will be inefficient in terms of computations and power consumption. In IOTA, PoW needs to be done for each transaction, and there are multiple transactions created in the same bundle, especially in the case when the amount of tokens that need to be transferred from one account to another account is split among multiple addresses owned by the sender's account. Then, PoW is done before sending bundle to the Tangle. Once the bundle is prepared, it is then sent to the network. Therefore, If an IOTA node installing Trinity wallet does not have enough capacity of computation, it cannot send transactions. What IOTA has done to solve this problem is called remote PoW which is not available in other blockchain systems. Considering the fact that not all machines have the computational capacity to do proof of work, IOTA has provided the capabilities to offload the tasks of computing PoW to remote nodes. This feature can be configured in the Trinity Wallet. However, these actions make the bundle preparation time to be larger.
%
%\item[Storage data retention:] Bitcoin does not support deleting history of the transactions. Hence, it suffers from ever increasing of the data size on the storage. Although, Ethereum and Hyperledger Fabric have introduced solutions (presented in Section~\ref{sec:datastorage}) for deleting state data from their database, the inherent feature of immutability (as one of the five pillars discussed in Section~\ref{sec:properties}) avoids any deletion from their transaction history. Even IOTA which uses snapshots for deleting history of transactions needs to keep the whole history of data in its permanodes to be used for some further verifications. Therefore, data storage capacity of blockchain nodes is a critical issue especially in public blockchains which are open to be accessed by unlimited number of users. The idea of sharding~\cite{sharding} is so far one of the most practical solutions to achieve a scale-out system where the storage, communication, and data manipulation can be divided among the participants. Elastico~\cite{elastico}, OmniLedger~\cite{omniledger}, and Rapidchain~\cite{rapidchain} are research examples that have been conducted in this area. 
%
%\item[Decentralization, security or scalability:] In addition to the storage scalability problem, ever growing of Tangle in IOTA makes a transaction verification inefficient. The reason is that the IOTA transaction issuer has to verify the whole history of a transaction in the large size Tangle. Centralized Coordinator of IOTA foundation (described in Section~\ref{sec:datamanipulation}) has solved this problem. IOTA Coordinator provides both security and efficiency of IOTA consensus protocol, and scalability of IOTA data storage. However, the Coordinator implementation rises the problem of centralization which can affect the blockchain participants' observation in terms of the system trustworthy. Hyperledger Fabric has the concept of private administrator organizations as well which are controlling membership of the participants and the network policies that makes Hyperledger Fabric a semi-centralized system. Hence, Achieving full degree of decentralization, security, and scalability may not be possible all together. This trade-off should be considered in developing a blockchain system. 
%
%\item[Number of consensus participants vs. throughput:] It has been observed in Section~\ref{sec:datamanipulation}) that consensus protocol in permissionless blockchains like Bitcoin, Ethereum, and IOTA is based on the activity of every node interested in participation. This mechanism has increased the consensus security of public blockchains since they will be independent of individual malicious decisions. However, public consensus mechanisms reduce throughput of such blockchain systems. On the other hand, Hyperledger Fabric as a permissioned blockchain system includes a limited number of participants in the consensus protocol to make the process faster, deterministic, and under control. This mechanism works quite efficient with few number of organizations participating in the consensus protocol, but as federation of organizations increases, the throughput will be decreased. Therefore, number of consensus participants and the consensus protocol type affects throughput of the blockchain systems. These parameters should be chosen wisely according to the use case of the blockchain.
%
%\item[Consensus flow:] Among the representative blockchain systems, transaction inclusion into the blockchain is deterministic only in Hyperledger Fabric. The reason of this difference is that the flow of consensus is different between Hyperledger Fabric and other presented public blockchains. In Hyperledger Fabric, agreement on inclusion of a block is happened before adding the block to the ledger. This means that all the validation process happens before adding the block to the ledger. The transactions and blocks validated and confirmed in the last phase of Hyperledger Fabric consensus protocol, they are never revoked, and they will be final in the blockchain. On the other hand, in public blockchains, confirming inclusion of the block and transactions are performed after adding them into the ledger. In this case, consensus will be probabilistic and based on the depth of the data item in the ledger. 
%
%\item[Event emission:] Events declared in Ethereum contracts are only for logging transactions. Although IOTA has not the concept of smart contracts, it introduces event emission in its account object. IOTA accounts can listen for events such as making or receiving a payment and log them to the user's console. Bitcoin can also enable the feature of event logging by external applications. However, chaincodes in Hyperledger Fabric supports registering and emitting special events inherently. Event services in Hyperledger Fabric have more functionalities than deployed on other representative blockchain systems as they affect both ledgers and database. They are stored on blockchain and are accessible using address of the contract till the contract is present on the blockchain. In addition to sending transactions logs, Hyperledger Fabric event service can send entire blocks that have been committed to the ledger If the related events are set by a chaincode.
%
%\item[Type of transaction:] While Bitcoin, Ethereum, and IOTA transactions are all related to the application functionality of these blockchain systems, Hyperledger Fabric introduces another type of transaction called configuration update transaction~\cite{configurationtx}. Configuration update transactions are used for updating a Hyperledger Fabric channel configuration such as changing the structure by adding members, or updating processes by modifying channel policies. On the other hand, represntative permissionless blockchain systems handle configuration updates by creating new forks in their blockchain systems.  

%\end{description}.?..
